The PEPSI Exoplanet Transit Survey (PETS) IV: Assessing the atmospheric chemistry of KELT-20b

Most ultra hot Jupiters (UHJs) show evidence of temperature inversions, in which temperature increases with altitude over a range of pressures. Temperature inversions can occur when there is a species that absorbs the stellar irradiation at a relatively high level of the atmospheres. However, the species responsible for this absorption remains unidentified. In particular, the UHJ KELT-20b is known to have a temperature inversion. Using high resolution emission spectroscopy from LBT/PEPSI we investigate the atomic and molecular opacity sources that may cause the inversion in KELT-20b, as well as explore its atmospheric chemistry. We confirm the presence of Fe I with a significance of 17$\sigma$. We also report a tentative $4.3\sigma$ detection of Ni I. A nominally $4.5\sigma$ detection of Mg I emission in the PEPSI blue arm is likely in fact due to aliasing between the Mg I cross-correlation template and the Fe I lines present in the spectrum. We cannot reproduce a recent detection of Cr I, while we do not have the wavelength coverage to robustly test past detections of Fe II and Si I. Together with non-detections of molecular species like TiO, this suggests that Fe I is likely to be the dominant optical opacity source in the dayside atmosphere of KELT-20b and may be responsible for the temperature inversion. We explore ways to reconcile the differences between our results and those in literature and point to future paths to understand atmospheric variability.

==> Comments.tex <==
We thank the referee for their careful reading of our paper. We have interspersed their comments with our responses below. We have marked all additions to the text of the paper in bold, and removals with strikethroughs, except for the correction of minor typos and grammatical errors which did not affect the meaning of the text.

Major comments:
Page 2; L9ff, left col.: This paragraph in the introduction deals with the TiO and VO conundrum in emission and transmission from a historical perspective. In recent months, additional work on this matter has been published, and I suggest the authors have a closer look at this paragraph again.
Notably, the work of Hoeijmakers et al. (2020) is at high spectral resolution and does not detect VO, but predicting its presence provided equilibrium chemistry with vanadium. Pelletier et al. (2023) recently reported the detection of VO at high spectral resolution in transmission with MAROON-X and ESPRESSO independently. 
I suggest adding that reference to convey the full picture. This also links to the conclusion, where the topic is brought up again, see comment Page 11, L47ff.

We have added more clarification on previous work searching for VO signals in high and low resolution, including adding the Pelletier et al. 2023 detection of VO in transmission with ESPRESSO and MAROON-X.

Page 2; L47ff, right col.: The methodology follows Johnson et al. (2023), creating a master spectrum (median) that is removed from all exposures (removing the stellar and time-independent components). The removal is done by subtracting the master spectrum from each spectrum in the time series. I would like to ask the authors to specify if the spectra of the time series have been normalised to a common flux level at this point. This, in turn, would make it valid to assume that subtraction and division yield the same to first order. Specifically, if the normalisation is done earlier, I recommend mentioning that in the text. In general, I recommend removals through divisions and not subtractions.

We have clarified in the text that the spectra are continuum-normalized to unity by the PEPSI pipeline well in advance of the median removal.

We have tried both median subtraction and median division. Empirically, median division performs worse for our data; using division rather than subtraction reduces the significance of the Fe I detection from 17 $\sigma$ to 8 $\sigma$.

Page 3, L50ff, right col.: To determine the abundance of each chemical species in the planet's atmosphere given the p-T profile, the authors use FastChem. FastChem computes the abundances as a function of altitudes. I'd like to ask the authors to clarify why they opt for a constant VMR (extracted at 1 bar). Is the expected VMR roughly constant over the full range of altitudes? If so, one could show that in a plot of VMRs. If not, what is the reason to opt for 1 bar?

We adopt a constant VMR as a function of altitude partly as a simplifying assumption, and partly as in reality there should be some amount of convection and diffusion in the atmosphere which should smooth out chemical gradients. As the focus of the current paper is simply on the detection of species, and not on a more careful retrieval of abundances (which we will pursue in future works) we believe that this simplifying assumption is appropriate to the current work.

Our FastChem models suggest that the abundances of the species in question should be approximately constant below the inversion, and only change at and above the location of the inversion at a few mbar. Additionally, assuming the presence of convection, the pressure level at which the abundances will be homogenized will not necessarily be at the photosphere.


Page 5, Table 2: I really appreciate Table 2 summarising all the results, but do have a question I suggest addressing in the caption or even in the text: How is the sigma of the injection recovery test computed? It seems to be the case that the injected recovery SNR is a lot stronger than the actual observed signal.

We added clarification to how the significance of the injection recovery tests were computed as well as explained why the significance of these tests are higher than the significance we see with our actual data.

Page 7, L50ff, left col.: To compare the significance of the injection recovery test and the actual observed significance, I recommend showing both panels for all the species together. This could all be done together in Figure 3 for both (tentative) detections (Fe I, Ni I). Additionally, it may be helpful to show the predicted line strength through a cut at the expected orbital velocity (one-dimensional cut instead of a two-dimensional panel).

We added the injection-recovery tests for Fe I and Ni I to visually compare the difference between their significance.

Page 8, L51ff: I appreciate the discussion of the non-confirmation/-detection of Fe II and Cr I compared to recent work. The authors use both molecfit (for telluric correction) and also SYSREM to correct for residual systematics. Could the authors comment on the impact of adding SYSREM to the analysis in terms of “eating away” signal of the planet? Is this something that could be assessed?

While it is true that SYSREM can attenuate the signal from the planet if too many systematics are removed, our extensive tests in Johnson et al. (2023) indicated that 1-3 systematics removed (after the use of Molecfit) result in the strongest detections (and that Molecfit+SYSREM results in better signal recovery than either Molecfit or SYSREM alone), and thereafter the signal is attenuated. We use no more than 3 systematics removed in this work, which should not strongly attenuate the signals. We use many fewer systematics than some works, e.g. Gibson et al. (2022) removed 15 systematics from their data, while Nugroho et al. (2017) removed 10. Our lower number of systematics removed compared to many other published works should result in less attenuation.



Page 10, Figure 6: Same as for Figure 3, I recommend adding the panels for the injection recovery test to this figure, see comment for Page 7, L50ff, left col. This allows merging Figures 6 and 7, while at the same time adding the injection recovery panel for Fe II.

We added the injection-recovery test for Fe II and combined figures 6 and 7.

Page 11, L47ff, right col.: Recently, Pelletier et al. (2023) detected VO in the transmission spectrum of WASP-76 b using both MAROON-X and ESPRESSO data. This strongly suggests that the line list is accurate enough to detect VO. Notably, the line list is known to become less accurate beyond 1 micron but not necessarily at optical wavelengths. I suggest adding this citation to the discussion.

We added the Pelletier et al. citation to our discussion as well as added insight about the accuracy of molecular line lists in optical wavelengths.

Small comments:
Page 2, L1: In this paragraph, the authors mention Kirchhoff’s Laws referring to Kirchhoff’s Law of thermal radiation. It may be interesting to add a citation (not necessarily to the Kirchhoff paper from 1860, but some more recent work) or write the full name of the law for clarity.

We changed this sentence to clarify that we are using Kirchhoff's Law of thermal radiation.

Page 2; L29ff, left col.: The paragraph introduces the system (stellar and orbital parameters). I suggest adding the equilibrium temperature of the planet for fast comparison to other ultra-hot Jupiters.

We added the thermal equilibrium temperature of KELT-20b for quick comparison with other hot ultra-hot Jupiters.

Page 3, L23ff, left col.: In the cross-correlation analysis, the weighting of the CCF is described as follows “These CCFs are combined in a weighted sum, in which the weights are the 95th percentile SNR from the chosen arm […] multiplied by the total equivalent width in the model emission lines within that bandpass.” The description is not entirely clear to me, and I ask the authors to clarify or cite the source of their weighting algorithm.

This approach was originally used by Johnson et al. (2023). The idea is to weight the CCFs by both the signal-to-noise and the information content of each arm for a given species. We have rewritten the text to clarify.

Page 3, L44ff, right col.: The p-T profile of the atmosphere used to model the cross-correlation templates is the same as in Johnson et al. (2023) but not shown in this manuscript. I suggest adding a figure with the profile to avoid skipping back to Johnson et al. (2023) to estimate the temperatures at different altitudes.

We have added a figure showing the P-T profiles, which is now Fig. 1 of the paper.

Page 4, L7, right col.: I suggest changing “we wanted to assess” to “we assessed”.

We changed "we wanted to assess” to “we assessed”.

Page 6, Figure 2: Figure 2 shows the model spectra of the notable atomic and molecular species treated in this study. I suggest increasing the font size of labels, tick labels and text in the plots in all the panels to increase readability.

We updated all of the font sizes Figure 2 to ensure maximum readability.

Page 7, Figure 3: Please add in the caption a description of the vertical and horizontal dashed lines.

We added clarification for the significance of vertical and horizontal in all CCF map figures.

Page 9, Figure 5: The caption of Figure 4 still includes a comment for a co-author to replace plots.

(Now Figure 6) All unnecessary text was removed from the caption and the figure was updated to include the correct alias plots.

Page 9, L44, right col: I suggest replacing “throwing out” with “removing”.

We replaced “throwing out” with “removing”. 

General comments: MaroonX should be spelled as MAROON-X.
I recommend increasing the font size of tick labels and axis labels to increase readability. Especially Figure 2

MAROON-X is now labeled correctly throughout the text.
Font size is addressed under "minor comments".

We also added a few additional brief comments in the main text requested by co-authors, and fixed a few minor typos.

